A Credit Assignment Compiler for Joint Prediction

Many machine learning applications involve jointly predicting multiple mutually dependent output variables. Learning to search is a family of methods where the complex decision problem is cast into a sequence of decisions via a search space. Although these methods have shown promise both in theory and in practice, implementing them has been burdensomely awkward. In this paper, we show the search space can be defined by an arbitrary imperative program, turning learning to search into a credit assignment compiler. Altogether with the algorithmic improvements for the compiler, we radically reduce the complexity of programming and the running time. We demonstrate the feasibility of our approach on multiple joint prediction tasks. In all cases, we obtain accuracies as high as alternative approaches, at drastically reduced execution and programming time.

==> Makefile <==
#all: l2s_nips16.pdf
all: nips_submission.pdf nips_supplement.pdf

l2s_nips16.pdf: l2s_nips16.tex
	pdflatex l2s_nips16.tex
	bibtex l2s_nips16
	pdflatex l2s_nips16.tex
	pdflatex l2s_nips16.tex	
nips_submission.pdf: l2s_nips16.tex
	cp l2s_nips16.tex nips_submission.tex
	sed -i 's/\\appendix/\\end{document}/' nips_submission.tex
	pdflatex nips_submission
	bibtex nips_submission
	pdflatex nips_submission.tex
	pdflatex nips_submission.tex

imperative_searn.pdf: imperative_searn.tex
	pdflatex imperative_searn.tex

nips_supplement.pdf: l2s_nips16.pdf
	pdftk l2s_nips16.pdf cat 10-end output nips_supplement.pdf

clean:
	rm l2s_nips16.pdf nips_submission.pdf

